Learning Skills to Patch Plans Based on Inaccurate Models

Planners using accurate models can be effective for accomplishing manipulation tasks in the real world, but are typically highly specialized and require significant fine-tuning to be reliable. Meanwhile, learning is useful for adaptation, but can require a substantial amount of data collection. In this paper, we propose a method that improves the efficiency of sub-optimal planners with approximate but simple and fast models by switching to a model-free policy when unexpected transitions are observed. Unlike previous work, our method specifically addresses when the planner fails due to transition model error by patching with a local policy only where needed. First, we use a sub-optimal model-based planner to perform a task until model failure is detected. Next, we learn a local model-free policy from expert demonstrations to complete the task in regions where the model failed. To show the efficacy of our method, we perform experiments with a shape insertion puzzle and compare our results to both pure planning and imitation learning approaches. We then apply our method to a door opening task. Our experiments demonstrate that our patch-enhanced planner performs more reliably than pure planning and with lower overall sample complexity than pure imitation learning.

==> results.tex <==
% First, we show which states tend to be marked as where the transition model is unreliable, and what unexpected observations occur. 
In this section, we describe the experiments used to evaluate our proposed method of combining model-based planning and model-free skill learning.
%First, we describe additioanal execution details and our baseline methods. We then present quantitative results that show how our method helps execution reliability and data efficiency over the baseline methods. Next, we investigate how the number of training samples effects the performance and reliability of our method.
For both tasks, the action is a 3D translation $\Delta x$ of the end-effector in the world frame and a rotation represented using a quaternion.%  \cite{scikit-learn}. 

\subsection{Experimental Setup}
\label{sec:experimental}
\textbf{Shape Insertion Setup:} The experimental setup for the shape insertion experiment is shown in Figure~\ref{fig:envsetup}. We use a children's 8-piece knob puzzle (or \textit{board}) mounted at a fixed location. The puzzle pieces are manipulated by a 7 DoF Franka Panda arm towards their respective goal locations. A 7cm x 8cm x 4cm PLA obstacle is placed in a location that obstructs any straight line paths to the goal for the indicated trials. The obstacle is never placed directly over the goal position.
For 3D object pose estimation, we attached AprilTags~\cite{apriltag} to the top of the puzzle pieces, obstacles, and at the goal locations. An overhead Microsoft Azure Kinect sensor is used to retrieve images of the scene. A second Azure Kinect sensor records downward angled images of the scene as input to the autoencoder described in Section~\ref{sec:overall}. 
The Franka arm indirectly estimates end-effector forces and torques using the joint torques. Force detected relative to the end-effector is converted into a binary signal by setting a force threshold that detects contact with objects, but does not trigger during acceleration for movement in free space. 

%We elaborate on the door opening task at the end of Section~\ref{sec:ExperimentalResults} and~\ref{sec:discussion}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{imgs/demophoto_option2.png}
    \caption{Demonstration where the human operator moves the robot arm, via teleoperation, to complete the shape insertion task after model failure. We found that demonstrations worked best when the operator reset the shape to a position outside of the hole and performed a sliding motion into the hole.}
    \label{fig:demosetup}
    \vspace{-1.5em}
\end{figure}

\textbf{Baselines:} We compare our method to two different baselines. The first is the planner described in Section~\ref{sec:model-based-planner}. For the second baseline, we learned a policy using Imitation Learning (IL) in conjunction with Dynamic Movement Primitives (DMPs)~\cite{kroemer2016meta, schaaldmp}. For the DMP baseline, initial grasping is performed using the planner. The transport and insertion are done with DMPs. The DMP for this task was trained by collecting a trajectory using a kinesthetic human demonstration, while the obstacle was obstructing the path to the goal. More specifically, the DMP was trained from the oval starting position using the rectangle puzzle piece as the manipuland. Each translational Cartesian dimension was modeled as a separate DMP component. We used the formulation shown in Eq.~\ref{eq:dmp} and~\ref{eq:dmpforce}. We use the modification mentioned in Section IV-A of~\cite{kroemer2016meta} to include a goal state parameter that scales the DMP trajectory towards the goal state. This formulation also allows for the use of object features that can be used to scale the amplitude of a trajectory. This is useful if the start and end positions are close to one another, since the trajectory's amplitude can become sensitive to the goal state parameter's scaling. We scaled the $z$ dimension trajectory by 0.5 to quell this issue. The DMP parameters for execution are learned through linear ridge regression.% Our approach also uses the planner for initial grasping and is described in Section~\ref{sec:approach}. 
\vspace{-1.5em}

\begin{equation}
    \vec{y}=\alpha_{z}\left(\beta_{z} \tau^{-2}\left(y_{0}-y\right)-\tau^{-1} \dot{y}\right)+\tau^{-2} \sum_{j=1}^{M} \phi_{j} f\left(x ; \boldsymbol{w}_{j}\right)
    \label{eq:dmp}
\vspace{-1em}
\end{equation}

\begin{equation}
    f\left(x ; \boldsymbol{w}_{j}\right)=\alpha_{z} \beta_{z}\left(\frac{\sum_{k=1}^{K} \psi_{k}(x) w_{j k} x}{\sum_{k=1}^{K} \psi_{k}(x)}+w_{i 0} \psi_{0}(x)\right)
    \label{eq:dmpforce}
\vspace{-0.5em}
\end{equation}

% For training, the human operator is notified, via computer console, when model failure is detected. The operator then assists in completing the task by moving the arm to the goal location through keyboard teleoperation. Images from the downward-angled Azure Kinect are collected as the demonstrations are performed. Examples of these images are shown in Figure~\ref{fig:demosetup}.

%\begin{outline}
%    \1 What we want to show in the experiments
%        \2 What states tend to be marked as where the transition model unreliable? What causes the unreliably?
%        \2 Is our method helping execution reliability?
%        \2 Is our method helping data efficiency?
%        \2 How does the number of training samples effect performance? How many are needed for a significant reliability increase?
%
%    \1 Experimental setup

%(this doesn't seem necessary) An example is shown in the rightmost photo of Figure ~\ref{fig:failureexamples}.

% \begin{figure}
% % \missingfigure[0.3\textwidth]{plot GP with 1.96\sigma confidence interval}
% \includegraphics[width=0.36\textwidth]{imgs/gpplot.png}
% \centering
% \caption{GP estimate of where $\widetilde{S}$ is in the $z$ axis in the shaded region.}
% \label{fig:GP}
% \end{figure}

%    \1 Which states tend to be unreliable?
%        \2 What do they look like? Walk through examples. (Figure ~\ref{fig:failureexamples})

%        \2 Where are they physically located? (Figure ~\ref{fig:uncertainregions})
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.4\textwidth]{imgs/badandgoodpoints.png}
%     \caption{Spatial 3-D graph of state space where model-error is high (red dots) and low (green dots) for the shape insertion task. The origin is the base of the robot and dimensions are in meters.}
%     \label{fig:uncertainregions}
% \end{figure}
%            \3 Close to the object, where the planner usually reaches it from. Good, because planner specific, but if diverse knowledge is needed, can take diverse samples during training
%        \2 Does this depend on the underlying policy? Does more funnelling behaviour change which states are considered bad for the transition model? (Only relevant if we do conCERRT)

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{imgs/barn}
    \vspace{-1.5em}
    \caption{Real world shape insertion results of all trials. The figure shows the number of times an outcome occurred for each implementation when there was no obstacle obstructing the path. Section~\ref{sec:ExperimentalResults} defines success.}
    \label{fig:successshape}
    \vspace{-1.5em}
\end{figure}

\subsection{Experimental Results}
\label{sec:ExperimentalResults}
In this section, we show how our method compares to the baseline methods described in Section~\ref{sec:experimental} on two real-world tasks. The first task is to insert a puzzle piece into its corresponding hole. The experiments are performed with three shapes: a rectangle, a circle, and a square. Each shape goes into one of 8 corresponding slots in a $4\times2$ grid, shown in the bottom left of Figure~\ref{fig:pybullet}. We perform 7 trials for each shape where the starting position is one of the 8 regions, excluding the goal region. These experiments are then repeated with an obstacle obstructing the straight line path from start to goal. Success occurs when the shape is completely in the hole, see the bottom right of Figure~\ref{fig:demosetup}. A partial success is when only part of the shape is in the hole, see Figure~\ref{fig:failureexamples}. Failure indicates that either the robot hit an obstacle during execution or the shape was not in the hole at all. 
% Each of the three approaches performed the shape insertion task for 20 trials with no obstacles obstructing their trajectories and for another 5 trials with an obstacle in their path. For our method and for the planner, we place the block in a different starting location each time. 
% We start the task once the robot makes contact with the shape, i.e. when the robot grasps the shape for shape insertion. 
% We define success as placing the entirety of the puzzle piece inside the target hole, partial success as having only a portion of the puzzle piece in the target hole, and failure as complete misalignment with no part of the puzzle piece entering the hole. 
We show the performance of our method after training, as well as the baseline performances, in Figure~\ref{fig:successshape}. The results for the trials with an obstacle are shown in Figure~\ref{fig:obstacleshape}. 

\begin{figure}[t]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.4\textwidth]{imgs/barwithobs.pdf}
    \vspace{-1.5em}
    \caption{Real world shape insertion results of all trials with an obstacle obstructing the path. The figure shows the number of times an outcome occurred for each implementation. Success is defined in Section~\ref{sec:ExperimentalResults}.}
    \label{fig:obstacleshape}
\end{figure}

\begin{figure}[t]
    \centering
    \begin{tabular}{ c|c|c|c|c }
      \# Expert Demos: &1 & 5 & 10 & 20 \\
      \hline
      Success Rate: &$7/21$ & $15/21$ & $16/21$  &$19/21$ \\
    \end{tabular}
    \caption{Overall success of our method on the shape insertion task depending on the number of training samples. The first row is the number of training samples used and the second row is the rate of success for the 21 trials. Success and the experimental trials performed are explained in~\ref{sec:ExperimentalResults}}.
    \label{fig:sampleeffect}
    \vspace{-1.5em}
\end{figure}

For the 21 shape insertion trials without the obstacle, we found that the method using the planner was only able to completely insert the puzzle pieces once, which occurred with the circle shape. The failure rate was $5/21$ and the partial success rate was $15/21$. The DMP baseline had a success rate of $4/21$, partial success rate of $15/21$, and failure rate of $5/21$. Lastly, our method had a success rate of $19/21$, partial success rate of $2/21$, and failure rate of $0/21$ when trained on 20 samples.

The next set of experiments show how well each method generalizes when an obstacle is introduced. The DMP method generates trajectories that collided with the obstacle $13/21$ times. Failures occur because the DMP parameters learned do not generalize over all possible obstacle configurations and starting locations. It should also be noted that the robot's joint configuration before the DMP was executed, i.e. the joint positions after the planner finished executing, seemed to affect the DMP's performance. We believe this was due to the goal configuration approaching the robot's joint limits from certain starting configurations. 

The method utilizing the planner hit the obstacle two times. This occurred when the task was constrained to a small area, causing the trajectory to go close to the obstacle and making the 1 cm perception error become more significant. An example of this is shown in Figure~\ref{fig:pybullet}. Our method, which relies on the planner for obstacle avoidance for most of the trajectory, also hits the obstacle $2/21$ trials. The remaining trials show performance similar to the trials without an obstacle, with a $16/21$ success and $3/21$ partial success rate. 
    
We also tested what effect using more trajectory demonstrations to train our method had on success rate. We observed an increase in success rate of insertion when more demonstrations were used. This is expected since the smaller $|\widetilde{\mathcal{D}}|$ is, the smaller the predicted region of $\tilde{S}$ becomes. Furthermore, more demonstrations lead to a better quality $\piMF$. These results are shown in Figure~\ref{fig:sampleeffect} and were performed without an obstacle.

\input{Sections/doordemo}
